Cer-Eval: Certifiable and Cost-Efficient Evaluation Framework for LLMs

As foundation models continue to scale, the size of trained models grows exponentially, presenting significant challenges for their evaluation. Current evaluation practices involve curating increasingly large datasets to assess the performance of large language models (LLMs). However, there is a lack of systematic analysis and guidance on determining the sufficiency of test data or selecting informative samples for evaluation. This paper introduces a certifiable and cost-efficient evaluation framework for LLMs. Our framework adapts to different evaluation objectives and outputs confidence intervals that contain true values with high probability. We use ``test sample complexity'' to quantify the number of test points needed for a certifiable evaluation and derive tight bounds on test sample complexity. Based on the developed theory, we develop a partition-based algorithm, named Cer-Eval, that adaptively selects test points to minimize the cost of LLM evaluation. Real-world experiments demonstrate that Cer-Eval can save 20% to 40% test points across various benchmarks, while maintaining an estimation error level comparable to the current evaluation process and providing a 95% confidence guarantee.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/main_result.tex <==
% \begin{table*}[t!]
% \footnotesize
%     \centering
%     % \vspace{-0.25in}
%     \caption{Comparison of our proposed Adaptive Sampling method with two baselines: IID Sampling and IRT Sampling. Results are reported across five datasets, i.e., MMLU, HELM, MMMU, HEIM, DecodingTrust, which covers a variety of LLM tasks including reasoning, multimodal understanding, and safety. We evaluate four SOTA models, i.e., Llama3.2-70B, InternVL2-40B, GPT-4o, OpenAI-o1 over four metrics, i.e., \textbf{SSR} (sample size ratio), \textbf{Err} (overall estimation error), \textbf{Avg Err} (estimation error averaged over subsets), and \textbf{Cost}, which is evaluated by the averaged time per subset. The best performance is in bold.}
%     \setlength{\tabcolsep}{1.2pt}
%     \resizebox{1.0\textwidth}{!}{
%     \begin{tabular}{l|c|cccc|cccc|cccc|cccc|cccc}
%         \toprule
%         \multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{4}{c|}{\bf MMLU} & \multicolumn{4}{c}{\bf HELM} &\multicolumn{4}{|c}{\bf MMMU} & \multicolumn{4}{|c}{\bf HEIM} & \multicolumn{4}{|c}{\bf DecodingTrust} \\
%         \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18} \cmidrule(lr){19-22}
%         & & SSR & Err. & Avg Err & Cost & SSR & Err. & Avg Err & Cost  & SSR & Err. & Avg Err & Cost & SSR & Err. & Avg Err & Cost & SSR & Err. & Avg Err & Cost \\
%         \midrule
%         \multirow{3}{*}{Llama3.2} 
%         & IID & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         & IRT & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         & \cellcolor{gray!30} \bf Adaptive & 
%         \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - \\
%         \midrule
%         \multirow{3}{*}{InternVL2}  
%         & IID & - & - & - & - & - & - & - & - & - 
%  & - & - & - & - & - & - & - & - & - & - & - \\
%         & IRT & - & - & - & - & - & - & - & - & -  & - & - & - & - & - & - & - & - & - & - & - \\
%         & \cellcolor{gray!30}  \bf Adaptive& 
%         \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - \\
%         \midrule
%         \multirow{3}{*}{GPT-4o}  
%         & IID & - & - & - & - & - & - & - & -  & - & - & - & - & - & - & - & - & - & - & - & - \\
%         & IRT & - & - & - & - & - & - & - & -  & - & - & - & - & - & - & - & - & - & - & - & - \\
%         & \cellcolor{gray!30} \bf Adaptive& 
%         \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - \\
%         \midrule
%         \multirow{3}{*}{OpenAI-o1}  
%         & IID & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
%         & IRT & - & - & - & - & - & - & - & - & - & - & - & -  & - & - & - & -  & - & - & - & - \\
%         & \cellcolor{gray!30}  \bf Adaptive& 
%         \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - & \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - &
%         \cellcolor{gray!30} - \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:main_result}
%     % \vspace{-0.25in}
% \end{table*}

\begin{table}[tb]
\footnotesize
    \centering
    \caption{Comparison of \ours with two baselines Base and Seq across three datasets (MMLU, AlpacaEval, MATH). Results are evaluated under estimation error level $\epsilon \approx 2\epsilon^* $ over two metrics: \textbf{SR} (saving ratio) and \textbf{FP} (empirical failure probability), both in percentage. The best performance is in bold.}
    % \setlength{\tabcolsep}{3pt}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|c|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{\bf MMLU} & \multicolumn{2}{c|}{\bf AlpacaEval} & \multicolumn{2}{c}{\bf MATH} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        & & SR & FP & SR & FP & SR & FP \\
        \midrule
        \multirow{3}{*}{Llama3.2-8B} 
        & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
        & Seq & 33.8 & 0 & 24.2 & 0 & 8.0 & 0 \\
        & \cellcolor{gray!30} \bf \ours & \cellcolor{gray!30} 38.4 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 38.1 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 20.8 & \cellcolor{gray!30} 0 \\
        \midrule
        \multirow{3}{*}{Mistral-7B}  
        & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
        & Seq & 33.8 & 0 &  24.2 & 0 & 8.0 & 0 \\
        & \cellcolor{gray!30} \bf  \ours & \cellcolor{gray!30} 33.7 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 62.3 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 51.7 & \cellcolor{gray!30} 0 \\
        \midrule
        \multirow{3}{*}{GPT-4o}  
        & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
        & Seq & 33.8 & 0 &  24.2 & 0 & 8.0 & 0 \\
        & \cellcolor{gray!30} \bf  \ours & \cellcolor{gray!30} 65.2 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 39.9 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 40.6 & \cellcolor{gray!30} 0 \\
        \midrule
        \multirow{3}{*}{Qwen2-7B}  
        & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
        & Seq & 33.8 & 0 &  24.2 & 0 & 8.0 & 0 \\
        & \cellcolor{gray!30} \bf  \ours & \cellcolor{gray!30} 42.4 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 71.5 & \cellcolor{gray!30} 0 & \cellcolor{gray!30} 29.2 & \cellcolor{gray!30} 0 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:main_result}
\end{table}

% \begin{table}[t!]
% \footnotesize
%     \centering
%     \caption{Comparison of \ours with two baselines Base and Seq across three datasets (MMLU, AlpacaEval, MATH). Results are evaluated under accuracy level $\epsilon \approx 2\epsilon^* $ over two metrics: \textbf{SR} (saving ratio) and \textbf{FP} (failure probability), both in percentage. The best performance is in bold.}
%     % \setlength{\tabcolsep}{3pt}
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{l|c|cc|cc|cc}
%         \toprule
%         \multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{\bf MMLU} & \multicolumn{2}{c|}{\bf AlpacaEval} & \multicolumn{2}{c}{\bf MATH} \\
%         \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%         & & SR & FP & SR & FP & SR & FP \\
%         \midrule
%         \multirow{3}{*}{Llama3.2-8B} 
%         & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
%         & Seq & 33.8 & 0.3 & 24.2 & 0.6 & 8.0 & 0.2 \\
%         & \cellcolor{gray!30} \bf \ours & \cellcolor{gray!30} 38.4 & \cellcolor{gray!30} 0.2 & \cellcolor{gray!30} 38.1 & \cellcolor{gray!30} 0.9 & \cellcolor{gray!30} 20.8 & \cellcolor{gray!30} 0.2 \\
%         \midrule
%         \multirow{3}{*}{Mistral-7B}  
%         & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
%         & Seq & 33.8 & 0.2 &  24.2 & 0.5 & 8.0 & 0.1 \\
%         & \cellcolor{gray!30} \bf  \ours & \cellcolor{gray!30} 33.7 & \cellcolor{gray!30} 0.2 & \cellcolor{gray!30} 62.3 & \cellcolor{gray!30} 1.3 & \cellcolor{gray!30} 51.7 & \cellcolor{gray!30} 0.5 \\
%         \midrule
%         \multirow{3}{*}{GPT-4o}  
%         & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
%         & Seq & 33.8 & 0.2 &  24.2 & 0.5 & 8.0 & 0.1 \\
%         & \cellcolor{gray!30} \bf  \ours & \cellcolor{gray!30} 65.2 & \cellcolor{gray!30} 0.3 & \cellcolor{gray!30} 39.9 & \cellcolor{gray!30} 1.1 & \cellcolor{gray!30} 40.6 & \cellcolor{gray!30} 0.3 \\
%         \midrule
%         \multirow{3}{*}{Qwen2-7B}  
%         & Base & 0 & 0 & 0 & 0 & 0 & 0 \\
%         & Seq & 33.8 & 0.3 &  24.2 & 0.5 & 8.0 & 0.1 \\
%         & \cellcolor{gray!30} \bf  \ours & \cellcolor{gray!30} 42.4 & \cellcolor{gray!30} 0.3 & \cellcolor{gray!30} 71.5 & \cellcolor{gray!30} 1.2 & \cellcolor{gray!30} 29.2 & \cellcolor{gray!30} 0.3 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:main_result}
% \end{table}
